Stable Energy Distribution of Weakly Dissipative Gasses under Collisional Energy Cascades

Collisional thermalization of a particle ensemble under the energy dissipation can be seen in variety of systems, such as heated granular gasses and particles in plasmas. Despite its universal existence, analytical descriptions of the steady-state distribution have been missing. Here, we show that the steady-state energy distribution of the wide class of collisional energy cascades can be well approximated by the generalized Mittag-Leffler distribution, which is one of stable distributions. This distribution has a power-law tail, as similar to Levy's stable distribution, the index of which is related to the energy dissipation rate. We demonstrate its universality by comparing Mont-Carlo simulations of dissipative gasses as well as the spectroscopic observation of the atom velocity distribution in a low-temperature plasma.

==> latexmkrc <==
#!/usr/bin/perl
$latex         = 'pdflatex %O -src-specials -shell-escape -interaction=nonstopmode -synctex=1 main';
$bibtex        = 'pbibtex %O %B';
$dvipdf        = 'dvipdfmx %O -o %D main_supplemental';
$pdf_mode      = 3; # use dvipdfmx

# Use SumatraPDF and atom inverse search
# $pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance -inverse-search "\"%USERPROFILE%\AppData\Local\atom\bin\atom.cmd\" \"%f:%l\"" %O %S';

# if you do not need to preview in -pvc option (preview document and countinuously update mode)
# $pdf_previewer = 'exit';

